Modeling Dynamics of Online Video Popularity

Large Internet video delivery systems serve millions of videos to tens of millions of users on daily basis, via Video-on-Demand and live streaming. Video popularity evolves over time. It represents the workload, as welll as business value, of the video to the overall system. The ability to predict video popularity is very helpful for improving service quality and operating efficiency. Previous studies adopted simple models for video popularity, or directly adopted patterns from measurement studies. In this paper, we develop a stochastic fluid model that tries to capture two hidden processes that give rise to different patterns of a given video's popularity evolution: the information spreading process, and the user reaction process. Specifically, these processes model how the video is recommended to the user, the videos inherent attractiveness, and users reaction rate, and yield specific popularity evolution patterns. We then validate our model by matching the predictions of the model with observed patterns from our collaborator, a large content provider in China. This model thus gives us the insight to explain the common and different video popularity evolution patterns and why.

==> sec/numerical.tex <==
\section{Numerical Solution}\label{Sec:num}

To better understand the evolution of videos' view count, we plot numerical values of $x(t)$, $dx(t)$
and $dw(t)$ in this section. We set total user population as fixed at $N=1,000,000$.

According to our model, $x(t)$ is the number of users who will view a particular video sooner or later.
$x(t)$ with two  evolution patterns is a key value to determine $dw(t)$.
We plot the evolution of $x(t)$ with $\alpha>\beta qN$ or $\alpha <\beta q N$ in Fig.~\ref{Fig:numxt}.
As we can see, the first type is a concavely increasing curve while the second type is a
convexly increasing curve before $t'$ and concavely increasing curve after $t'$.
\begin{figure}[ht]
\centering
\includegraphics[width=0.38\textwidth]{./fig/xt.eps}
\caption{ Evolution of $x(t)$ with $N=1,000,000$, $\beta=0.1/N$, $q=0.5$, $\alpha=0.00005 \text{ or }  0.1$ }
\label{Fig:numxt}
\end{figure}

Then, we plot the curve of $\frac{dx(t)}{dt}$ by setting
$\beta qN <\alpha< (2+\sqrt{3})\beta qN$,  $\alpha>(2+\sqrt{3})\beta qN$, $0<\alpha< (2-\sqrt{3})\beta qN$ or $(2-\sqrt{3})\beta <\alpha< \beta qN$
respectively in Fig.~\ref{Fig:numdx}. These results are consistent with our model with four different evolution patterns.
As $\alpha$ is relative small compared with $\beta qN$, curves of $\frac{dx(t)}{dt}$ have heavy tails.
\begin{figure}[ht]
\centering
\includegraphics[width=0.48\textwidth]{./fig/dx.eps}
\caption{ Evolution of $dx(t)/dt$ with  $N=1,000,000$, $\beta=0.1/N$, $q=0.05$, $\alpha = 0.00005 \text{ or } 0.0014 \text{ or } 0.0055\text{ or } 0.0188$.}
\label{Fig:numdx}
\end{figure}

The curve of $\frac{dx(t)}{dt}$ will significantly affect the evolution of $\frac{dw(t)}{dt}$, i.e., the evolution of view count.
We use the same parameters with Fig.~\ref{Fig:numdx} except $\gamma$.
In Fig.~\ref{Fig:numdwgh}, we set $\gamma=10$ a high value.
As one can observe, the evolution of $\frac{dw(t)}{dt}$ is almost the same with
that of $\frac{dx(t)}{dt}$,  which has been stated in Corollary~\ref{Coro:biggamma}.
In Fig.~\ref{Fig:numdwgl}, we set $\gamma = 0.001$ to get different evolution of $\frac{dw(t)}{dt}$.
Compared with Fig.~\ref{Fig:numdwgh},
with smaller $\gamma$ the peaks of $\frac{dw(t)}{dt}$ are delayed.

\begin{figure}[ht]
\centering
\includegraphics[width=0.48\textwidth]{./fig/dw_gamma_high.eps}
\caption{Evolution of $dw(t)/dt$ with $\gamma=10$ and other parameters the same with $dx(t)/dt$}
\label{Fig:numdwgh}
\end{figure}


\begin{figure}[ht]
\centering
\includegraphics[width=0.48\textwidth]{./fig/dw_gamma_low.eps}
\caption{Evolution of $dw(t)/dt$ with $\gamma  = 0.001$ and other parameters the same with $dx(t)/dt$}
\label{Fig:numdwgl}
\end{figure}

